Adaptive multiscale model reduction for nonlinear parabolic equations using GMsFEM

In this paper, we propose a coupled Discrete Empirical Interpolation Method (DEIM) and Generalized Multiscale Finite element method (GMsFEM) to solve nonlinear parabolic equations with application to the Allen-Cahn equation. The Allen-Cahn equation is a model for nonlinear reaction-diffusion process. It is often used to model interface motion in time, e.g. phase separation in alloys. The GMsFEM allows solving multiscale problems at a reduced computational cost by constructing a reduced-order representation of the solution on a coarse grid. In arXiv:1301.2866, it was shown that the GMsFEM provides a flexible tool to solve multiscale problems by constructing appropriate snapshot, offline and online spaces. In this paper, we solve a time dependent problem, where online enrichment is used. The main contribution is comparing different online enrichment methods. More specifically, we compare uniform online enrichment and adaptive methods. We also compare two kinds of adaptive methods. Furthermore, we use DEIM, a dimension reduction method to reduce the complexity when we evaluate the nonlinear terms. Our results show that DEIM can approximate the nonlinear term without significantly increasing the error. Finally, we apply our proposed method to the Allen Cahn equation.

==> _graphs_template.tex <==
%% 2 Sub-figures



%% END of 2 Sub-figures

%% 4 Sub-figures

% \begin{subfigure}{0.48\textwidth}
% \centering
% \includegraphics[width=1.0\linewidth, height = 5.5cm]{graphs/com_diff_on_enrich_08a.eps}
% \caption{$\theta = 0.8$, $\gamma = 0.8$, $\beta =0.8$ and $\tau = 0.8$.}
% \label{fig:goal_diffon_2}
% \end{subfigure}

% \begin{figure}[th]
% \mbox{
% \begin{subfigure}{0.48\textwidth}
% \centering
% \includegraphics[width=1.0\linewidth, height = 5.5cm]{graphs/com_diff_on_enrich_05.eps}
% \caption{$\theta = 0.5$, $\gamma = 0.5$, $\beta = 0.5$ and $\tau = 0.5$.}
% \label{fig:goal_diffon_3}
% \end{subfigure}

% \begin{subfigure}{0.48\textwidth}
% \centering
% \includegraphics[width=1.0\linewidth, height = 5.5cm]{graphs/com_diff_on_enrich_03.eps}
% \caption{$\theta = 0.3$, $\gamma = 0.3$, $\beta = 0.3$ and $\tau = 0.3$.}
% \label{fig:goal_diffon_4}
% \end{subfigure}
% }
% \caption{Comparing different online enrichments. ($l_i = 3$)}
% \label{fig:goal_diffon}
% \end{figure}

%% END of 4 Sub-figures



==> _table_template.tex <==
\begin{table}[h]
\caption{$L^2$-error with different source functions in Example 4.1.(S:Start, E:end)}. 
\centering
	\begin{tabular}{c|c|c|c|c|c}
	\hline \hline
		Source function& Online status &$ t=0.1$ & $t=0.2$ & $t=0.4$  & $t=0.8$\\
	\hline 
	    \multirow{2}{5em}{$f=1+u$} & $S$&$2.236\%$&$2.254\%$&$	2.255\%$&$2.255\%$\\
		        & $E$&$0.05839\%$&$0.05959\%$ &	$0.05968\%$ & $0.05968\%$\\
		\multirow{2}{5em}{$f=1+u^2$}& $S$&$2.228\%$&$2.246\%$&$	2.247\%$&$2.247\%$\\		
		 & $E$&$0.06204\%$ & $0.06140\%$ & $0.06140 \%$ &$0.06140\%$\\
		\multirow{2}{5em}{$f=1+u^3$} & $S$&$2.228\%$&$2.246\%$&$2.247\%$&$2.247\%$\\
		& $E$&$0.05949\%$&$0.06064\%$&$	0.06083\%$&$0.06213\%$	\\
	\hline
	\end{tabular}
\end{table}\\

\begin{table}[h]
\centering
\caption{The quantities using different numbers of basis functions}. 
	\begin{tabular}{c|c|c|c|c}
	\hline \hline
		Number of basis & $ t=0.1$ & $t=0.2$ & $ t=0.4$& $t=0.8$\\
	\hline 
		1 & $0.1910\%$&$ 0.1578\%$&$0.1617\%$&$0.1617\%$ \\
		2 & $0.06204\%$ & $0.06140\%$ & $0.06140 \%$ &$0.06140\%$\\
		3 & $0.06063\%$ & $0.05724\%$ & $0.05724\%$ &$0.05724\%$\\	
		4 & $0.04942\%$ & $0.05546\%$ & $0.05545\%$ &$0.05545\%$\\
		
	\hline
	\end{tabular}

\end{table}


\begin{table}[h]
\caption{The quantities under different initial conditions}. 
\centering
	\begin{tabular}{c|c|c|c|c}
	\hline \hline
		Initial Solution & $ t=0.1$ & $t=0.2$ & $ t=0.4$& $t=0.8$\\
	\hline 
	$u_1$	 & $0.05429\%$&$0.06822 \%$&$0.06825\%$&$0.06825\%$ \\
	$u_1$	 & $0.5430\%$ & $0.6823\%$ & $0.06825 \%$ &$0.06825\%$\\
	$u_1$	  & $0.5430\%$ & $0.6823\%$ & $0.06825 \%$ &$0.06825\%$\\	
	
		
	\hline
	\end{tabular}
	
	\label{tab:dual_importance}
\end{table}

